Byzantine Fault Tolerant Causal Ordering

Causal ordering in an asynchronous system has many applications in distributed computing, including in replicated databases and real-time collaborative software. Previous work in the area focused on ordering point-to-point messages in a fault-free setting, and on ordering broadcasts under various fault models. To the best of our knowledge, Byzantine fault-tolerant causal ordering has not been attempted for point-to-point communication in an asynchronous setting. In this paper, we first show that existing algorithms for causal ordering of point-to-point communication fail under Byzantine faults. We then prove that it is impossible to causally order messages under point-to-point communication in an asynchronous system with one or more Byzantine failures. We then present two algorithms that can causally order messages under Byzantine failures, where the network provides an upper bound on the message transmission time. The proofs of correctness for these algorithms show that it is possible to achieve causal ordering for point-to-point communication under a stronger asynchrony model where the network provides an upper bound on message transmission time. We also give extensions of our two algorithms for Byzantine fault-tolerant causal ordering of multicasts.

==> 01-Attacks.tex <==
\begin{section}{Attacks due to Byzantine Behaviour}

Each message $m$ sent to $p_i$ is accompanied with a \textit{logical timestamp} in the form of a matrix clock providing information about send and receive events in the causal past of $m$ denoted as $P(send(m))$. This is to ensure that all messages $m^\prime$ $\in$ $P(send(m))$ whose destination is $p_i$ are delivered at $p_i$ before $m$. The implementation as follows:

\begin{enumerate}
    \item Each process $p_i$ maintains a vector $Delivered$ of size $n$ with $Delivered_i[j]$ storing a count of messages sent by $p_j$ and delivered by $p_i$. 
    
    \medskip
    
    \item Each message $m$ has an associated a matrix timestamp $M^m_{sent}$, where $M^m_{sent}[i,j]$ stores a count of the number of messages sent by $p_i$ to $p_j$ as known to the sender of $m$ at the time of sending $m$. Each process maintains a matrix clock, $M_{sent}$.
    
    \medskip
    
    \item When message $m$ is received by $p_i$, it is not
    delivered until the following condition is met:
    
    
    
    \begin{center}
    
    $\forall k$, $M^m_{sent}[k,i] \leq Delivered_i[k]$
        
    \end{center}
    
    \medskip
    
    \item After delivering a message $m$, $p_i$ merges the logical timestamp associated with $m$ with its own matrix clock, $M^i_{sent}$.
    
  
\end{enumerate}


A Byzantine process may fabricate values in the matrix timestamp in order to disrupt the causal ordering of messages in an asynchronous execution. The attacks are described in the following subsections.

\subsection{Artificial Boosting Attack}

A Byzantine process $p_j$ may increase values of $M^j_{sent}[x,*]$ beyond the number of messages actually sent by process $x$ to one or more processes. When $p_j$ sends a message with such a Byzantine timestamp to any correct process $p_i$, it will result in $p_i$ recording Byzantine values in its $M_{sent}$ matrix. These Byzantine values will get propagated across correct processes upon further message passing. This will finally result in correct processes no longer delivering messages from other correct processes because they will be waiting for messages to arrive that have never been sent.   

As an illustrative example, consider a system of $n$ processes communicating by message passing. Let $(n-1)$ processes be correct and a single process be malicious - $p_j$. At the time of executing an artificial boosting attack, $p_j$ forges values in its $M_{sent}$ matrix as follows: if $p_j$ has sent $x$ messages to $p_k$, it can set $M^j_{sent}[j,k] = (x + d)$, $d >0$. When $p_i$ delivers a message from $p_j$, it sets 
$M^i_{sent}[j,k] = (x + d)$. Finally, when $p_i$ sends a message $m$ to $p_k$, $p_k$ will wait for messages to arrive from $p_j$ (messages that $p_j$ has never sent) before delivering $m$. This is because $(Delivered_k[j] \leq x)$ $\land$ $(M^m_{sent}[j,k] = x + d)$ $\Longrightarrow$ $(Delivered_k[j]  < M^m_{sent}[j,k])$. Therefore, $p_k$ will never be able to deliver $m$. A single Byzantine process $p_j$ has effectively blocked all communication from $p_i$ to $p_k$. This attack can be replicated for all pairs of processes by $p_j$. In another attack with a similar result, $p_j$ can increase $M^m_{sent}[k,i]$ to a \textit{near infinite} (very large) value and send $m$ to $p_i$. Once $m$ is delivered at $p_i$, $p_i$ will expect a very large number of messages to arrive from a correct process $p_k$ before delivering a message from any other process. In this way, liveness for process $p_i$ is disrupted.

In other words, a single Byzantine process can block all communication in an asynchronous message passing system which attempts to causally order messages.


\subsection{Safety Violation Attack}

A Byzantine process $p_j$ may decrease values of $M^m_{sent}[*,i]$ to smaller values than the true causal past of message $m$ and send it to a non-faulty process $p_i$. This may cause $m$ to get delivered out of order at $p_i$ resulting in a causal violation. Furthermore, if $p_j$ decreases the value of $M^m_{sent}[*,*]$ to smaller values than the true causal past of message $m$ then, once $m$ is delivered to $p_i$ and $p_i$ sends a message $m'$ to correct process $p_k$, there may be a further causal violation due to a lack of transitive causal data transfer from $m$ to $p_i$ prior to event $send(m')$. These potential causal violations are a result of the possibility of a message getting delivered before messages in its causal past at a common destination.

As an illustrative example, consider a system of $n$ processes communicating by message passing. Let $(n-1)$ processes be correct and a single process be malicious - $p_j$. At the time of executing a safety violation attack, $p_j$ forges values in its $M_{sent}$ matrix as follows: if $p_j$ knows that $p_k$ has sent $x$ messages to $p_i$, $p_j$ can set $M^m_{sent}[k,i] = x - 1$ and send $m$ to $p_i$.
If $m$ is received at $p_i$ before the $x^{th}$ message $m'$ from $p_k$ is delivered, it may get delivered before $m'$ resulting in a causal violation at $p_i$. In another attack, if $p_j$ knows that $p_l$ has sent $y$ messages to $p_k$, it can reduce $M^m_{sent}[l,k] = y -1$ and send $m$ to $p_i$. If $p_i$ delivers $m$ and sends $m'$ to $p_k$ before $m''$, the $y^{th}$ message from $p_l$, is delivered at $p_k$, $m'$ may get delivered before $m''$ resulting in a causal violation at $p_k$. In this way, a malicious process may cause causal violations at multiple correct processes by sending a single message with incorrect causal control information.




\end{section}

==> 02-Solution.tex <==
\begin{section}{Proposed Solution}

We propose point-to-point communication protocol that utilizes a modified version of Bracha's \textit{reliable Byzantine broadcast} \cite{bracha1985,bracha1987asynchronous} as an underlying abstraction. The broadcast ensures that all processes have correct and updated knowledge of each other processes' matrix clocks. The solution for Byzantine causal point-to-point messaging is presented in algorithm \ref{alg:bcb}. Algorithm \ref{alg:bcb} utilizes the br-broadcast() and br-deliver() primitives to make use of the reliable Byzantine broadcast implemented in algorithm \ref{alg:mbrb}. The application uses the bco-send() primitive to send causally ordered point-to-point messages and the bco-deliver() primitive delivers causally ordered messages to the application. 
Algorithm \ref{alg:bcb} assumes FIFO communication channels. The modified Byzantine reliable broadcast is specified in algorithm \ref{alg:mbrb}. Algorithm \ref{alg:bcb} stores casual information at each process in a three dimensional vector $M_i$. $M_i[j,*,*]$ is the matrix clock of $p_j$ stored at $p_i$. Specifically, $M_i[j,k,l]$ keeps track of the number of messages sent by $p_k$ to $p_l$ as known to $p_j$ stored at $p_i$. $Delivered_i$ is a vector stored at $p_i$ that counts the number of messages delivered from each other process. The count of messages sent by $p_j$ and delivered at $p_i$ is stored at $Delivered_i[j]$. 

The following is a categorization of the primitives used by algorithms \ref{alg:bcb} and \ref{alg:mbrb} for communication through message passing:

\begin{enumerate}
    \item \textbf{br-broadcast(m)}: Reliable broadcast that can withstand upto $t < n/3$ Byzantine nodes. Sends message $m$ to all processes using Bracha's 3 phase method.
    
    \medskip
    
    \item \textbf{br-deliver($m$,$i$)}: Delivers message $m$ sent via br-broadcast() primitive.
    
    \medskip
    
    \item \textbf{bco-send($m$,$i$)}: Sends message $m$ to process $p_i$ and informs all processes about the send event using the br-broadcast() primitive. 
    
    
    \medskip
    
    \item \textbf{bco-deliver($m$)}: Delivers message $m$ sent via the bco-send() primitive.
    
    \medskip
    
    \item \textbf{send($seq$,$m$,$i$)}: Sends message $m$ with sequence number $seq$ to process $p_i$ over a FIFO channel. Sequence number can be kept blank depending on the protocol.
    
    \medskip
    
    \item \textbf{receive($m$)}: Receives message $m$ sent via the send() primitive over a FIFO channel. 
\end{enumerate}

\medskip

\medskip


\begin{algorithm}[H]

\SetAlgoLined

\SetKwComment{Comment}{$\triangleright$ }{}
\KwData{Each $p_i$ maintains $M_i[1...n,1...n,1...n]$ and  $Delivered_i[1...n]$ with all values initialized to $0$}

\medskip

Each process $p_i$ for $0 \leq i < n$ executes the following: 

\medskip

\textbf{operation} $bco\_send(m,j)$ sends message $m$ to $p_j$:  \\

\Indp

$send(-,m,j)$  \\
$br \_ broadcast(\langle i,j,sent \rangle)$     \\
% $M[i,i,j] = M[i,i,j] + 1$   \\

\Indm

\medskip
    
\textbf{when} message $m$ is br$\_$delivered from $p_j$:

\Indp\While{$\exists x :Delivered_i[x] < M_i[j,x,i]$}{

wait in a non-blocking manner 

}
$bco\_deliver(m)$ \\
$br\_broadcast(\langle i,j,delivered \rangle)$  \\
% $M_i[i,*,*] = merge(M_i[i,*,*],M_i[j,*,*])$ \\
$Delivered_i[j] = Delivered_i[j] + 1$ 



\Indm

\medskip

\textbf{when} $\langle x,y,sent \rangle$ is br$\_$delivered from $p_x$:

\Indp

$M_i[x,x,y] = M_i[x,x,y] + 1$



\Indm

\medskip

\textbf{when} $\langle x,y,delivered \rangle$ is br$\_$delivered from $p_x$:

\Indp

$M_i[x,*,*] = merge(M_i[x,*,*], M_i[y,*,*])$



\Indm







 
 
\caption{Byzantine Causally Ordered point-to-point Protocol}
\label{alg:bcb}
\end{algorithm}


\begin{algorithm}[H]

\SetAlgoLined

\KwData{Each $p_i$ maintains a sequence number, $seq_i$ initialized to $0$}

\medskip

Each process $p_i$ for $0 \leq i < n$ executes the following: 

\medskip

\textbf{operation} $br\_broadcast(m)$: \\

\Indp

broadcast $init(i,seq_i,m)$ \\
$seq_i = seq_i + 1$

\Indm

\medskip

\textbf{when} $init(j,seq_j,m)$ is received:

\Indp

\If{$init(j,seq_j,m)$ is the first broadcast from $p_j$ with sequence number $seq_j$}{
    
    \medskip
    
    \If{$m[2] == i$ $\land$ $m[3] == sent$}{
    
    \If{message $m$ has been received from $p_j$}{
    
    broadcast $echo(j,seq_j,m)$
    
    }
    
    \ElseIf{message $m$ has \textbf{not} been received from $p_j$}{
    
    broadcast $veto(j,seq_j,m)$
    
    }
    
    }
    
    \medskip
    
    \ElseIf{$m[2] \neq i$ $\land$ $m[3] == sent$}{
    
    broadcast $echo(j,seq_j,m)$
    
    }
    
    \medskip
    
    \ElseIf{$m[2] \neq i$ $\land$ $m[3] == received$}{
    
    broadcast $echo(j,seq_j,m)$
    
    }
    
    \medskip
    
    \ElseIf{$m[2] == i$ $\land$ $m[3] == received$}{
    
        \If{$p_i$ has \textbf{not} sent message $m$ to $p_j$}{
    broadcast $veto(j,seq_j,m)$
    }
    
    
    \ElseIf{$p_i$ has sent message $m$ to $p_j$}{
    
    broadcast $echo(j,seq_j,m)$
    
    }
    
    }
    
    
}

\Indm

\medskip

\If{$init(j,seq_j,m)$ is received \textbf{and} $veto(j,seq_j,m)$ is received from $p_{m[2]}$}{

    \textbf{abort} broadcast


}

\medskip

\textbf{when} $echo(j,seq_j,m)$ is received do: \\

\Indp

\If{ $echo(j,seq_j,m)$ is received from more than $(n+t)/2$ processes $\land$ $ready(j,seq_j,m)$ has not been broadcast $\land$  $echo(j,seq_j,m)$ is received from $p_{m[2]}$}{

broadcast $ready(j,seq_j,m)$


}


\Indm

\medskip

\textbf{when} $ready(j,seq_j,m)$ is received:

\Indp

\If{$ready(j,seq_j,m)$ is received from $(t+1)$ processes $\land$ $ready(j,seq_j,m)$ has not been broadcasted}{

broadcast $ready(j,seq_j,m)$

\If{$m[3] == receive$ $\land$ the corresponding $send$ broadcast has not been delivered}{
Wait for send broadcast to get delivered

}


}

%\If{$ready(j,seq_j,m)$ is received from $(2t+1)$ processes $\land$ $(j,seq_j,m)$ has not been delivered $\land$ %$echo(j,seq_j,m)$ is received from $p_{m[2]}$ $\land$ $m[1] == i$}{
%    \textbf{deliver} $(j,seq_j,m)$ \\
%    %send $complete(seq_i)$ to all processes that have sent a ready message for $send_{seq_i}$

%}

\If{$ready(j,seq_j,m)$ is received from $(2t+1)$ processes $\land$ $(j,seq_j,m)$ has not been delivered $\land$   Broadcast with sequence number $seq_j -1$ from $p_j$ has completed locally}{

$br\_deliver(j,seq_j,m)$

}


\Indm




\caption{Byzantine Reliable Broadcast with Veto Mechanism}
\label{alg:mbrb}
\end{algorithm}

%-----------------------------------------------------------------------------------------------------------------

Algorithm \ref{alg:tpbv} presents a two phase broadcast algorithm that is used by algorithm \ref{alg:bcb} to increment matrix clocks at each process whenever a process sends or delivers a message. The aim of algorithm \ref{alg:tpbv} is to disseminate information whenever a single process makes a change to its clock and make sure that all \textit{correct processes} modify their clock whenever another correct process does so after a send/deliver event. Whenever $p_i$ sends a message to $p_j$, it informs all other processes via \textit{tp-broadcast} that it has sent a message to $p_j$. Processes wait for $p_j$ to confirm that $p_i$ has actually sent a message by waiting for an \textit{acknowledgement message} from $p_j$ before making changes to their clocks. The same is followed while receiving a broadcast following a deliver event. If process $p_i$ figures out that $p_j$ is exhibiting Byzantine behaviour by misinforming the system about send/deliver event concerning $p_i$, it send a \textit{veto message} terminating the broadcast at each other process. Each two phase  broadcast sends out message $c$. In case of a send broadcast, $c[0]$ is the sender, $c[1]$ is the receiver and $c[2]$ contains "sent". In case of a deliver broadcast, $c[0]$ is the receiver, $c[1]$ is the sender and $c[2]$ contains "received".

\medskip

\begin{algorithm}[H]

\SetAlgoLined

\SetKwComment{Comment}{$\triangleright$ }{}
\KwData{Each $p_i$ maintains a sequence number $seq_i$ initialized to $0$.}

\medskip

\textbf{operation} $tp\_broadcast(c)$: \\

\Indp

\For{all processes $p_x$}{

$send(seq_i,c,x)$ \\
$seq_i = seq_i + 1$
}

\Indm

\medskip

\textbf{when} message $c$ with sequence number $seq_j$ is received from $p_j$: \\

\Indp

\If{$c[1] == i$ $\land$ $c[2] == sent$ $\land$ $seq_j$ messages have arrived from $p_j$ $\land$ the $seq_j -1$ broadcast from $p_j$ has been $tp\_delivered$}{

$tp\_deliver($c$)$ \\

\For{all processes $p_x$}{

$send(\langle seq_j,j \rangle,ack,x)$ 
}


}



\If{$c[1] == i$ $\land$ $c[2] == delivered$ $\land$ $p_i$ has sent a message to $p_j$   $\land$ the $(seq_j -1)^{th}$ broadcast from $p_j$ has been $tp\_delivered$}{

$tp\_deliver(c)$ \\

\For{all processes $p_x$}{

$send(\langle seq_j,j \rangle,ack,x)$ 
}


}


\If{$c[1] \neq i$ $\land$ $seq_j$ messages have arrived from $p_j$ $\land$ the $(seq_j -1)^{th}$ broadcast from $p_j$ has been $tp\_delivered$}{

\If{$(\langle seq_j,j \rangle,ack)$ has not arrived from $p_{c[2]}$}{

wait for acknowledgement message from $p_{c[2]}$

}

$tp\_deliver(c)$ 



}


\Indm

 
\medskip
 
\textbf{when} $veto$ message with identifier $\langle seq_j,j \rangle$ is received from $p_{c[2]}$ $\land$ $c$ is the $seq_j^{th}$ broadcast from $p_j$:  \\

\Indp

abort broadcast initiated by $p_j$ with sequence number $seq_j$  

\Indm

 
\caption{Two Phase Broadcast with Veto}
\label{alg:tpbv}
\end{algorithm}




\end{section}

==> 03-Criteria.tex <==
\begin{section}{Correctness Conditions}



In order to be correct, any causal ordering algorithm for point-to-point messages must ensure the following:

\begin{enumerate}
    \item \textbf{Safety:} $\forall m' \in P(m)$, no correct process delivers $m$ before $m'$. 
    
    \medskip
    
    \item \textbf{Liveness:} All messages sent by non-faulty processes to non-faulty processes will be delivered eventually.
    
    
\end{enumerate}

%No message $m$ can be delivered at a non-faulty process if $\exists m' \in P(m)$ such that destination($m$) = destination %($m'$) and $m'$ has not been delivered.


\end{section}



==> 04-proof.tex <==
\begin{section}{Proof of Correctness}

\begin{lemma}
$\forall$ $i$ The local order of a correct process $p_i$ is observed at each correct process during the entire execution of algorithm \ref{alg:bcb}.

\label{lm:po1}

\end{lemma}

\begin{proof}

Each process informs every other process via a broadcast (as part of its send event) about a local send/receive event. The broadcast of the $x^{th}$ message completes locally at each process before the broadcast of the $(x+1)^{th}$ message. This is because in phase 3 of the broadcast specified in algorithm \ref{alg:mbrb} (line 31) each process checks to make sure that all broadcasts associated with prior events from the sending process are completed before any event's broadcast
is completed locally.

A Byzantine process may try to forge a broadcast for the $x^{th}$ event at process $p_i$ but such a broadcast will get vetoed at all correct processes locally, because they require consent from $p_i$ in the form of an $echo$ message, but will receive a $veto$ message (line 11/18)  instead

In this way, program order of send events at a correct process is preserved at all correct processes executing algorithm \ref{alg:mbrb}.



\end{proof}


\begin{lemma}
A send event by a correct process, $send(m)$ is observed before its corresponding receive event $rec(m)$, by each correct process in a system executing algorithm \ref{alg:bcb}.

\label{lm:po2}

\end{lemma}

\begin{proof}

In order to deliver a receive broadcast in algorithm \ref{alg:mbrb}, each process checks to make sure that the corresponding send broadcast has completed locally (line 30). Otherwise, the process waits for the send broadcast to complete before proceeding to check for the required messages in phase 3. 

A Byzantine process may send out a receive broadcast for a send message from a correct process that it never received, but such a  broadcast will never complete at any correct process because the correct process that supposedly sent the message will send a $veto$ message resulting in each correct process aborting the broadcast.


Therefore, causality between message sends and their corresponding receives is preserved in algorithm \ref{alg:mbrb}.  

\end{proof}


\begin{theorem}
The partial order of execution is observed at each correct process executing algorithm \ref{alg:bcb}.
\label{th:partial_order}

\end{theorem}

\begin{proof}

From lemmas \ref{lm:po1} and \ref{lm:po2}, we have the following:

\begin{enumerate}
    \item If $e^i$ and $e^j$ execute at the same correct process and $e^i$ executes before $e^j$, we have $e^i \rightarrow e^j$
    
    \medskip
    
    \item $\forall$ messages $m$ sent from and received at a correct process, $send(m) \rightarrow rec(m)$
    


\end{enumerate}
    
Transitively, we have a common partial order that is observed at each process.
    


\end{proof}

\begin{theorem}

The reliable broadcast algorithm given in algorithm \ref{alg:mbrb} is correct.

\end{theorem}

\begin{proof}

\end{proof}

\begin{theorem}{Algorithm \ref{alg:bcb} is correct while $t < n/3$.}

 







\label{Theorem:th1}

\end{theorem}

\begin{proof}

Algorithm \ref{alg:bcb} can tolerate at most $t < n/3$ Byzantine failures. This constraint arises from the underlying reliable broadcast primitive used for communicating control information.
This proof is divided into two parts - for failure free setting and for the Byzantine setting. Assuming the failure free model, we have:

\begin{itemize}
    
    
    \item \textbf{Safety:}
    
    \medskip
    
    \item \textbf{Liveness:} When message $m$ sent by $p_i$ is received at process $p_j$, it is either delivered before any other message or it may end up waiting to get delivered because $\exists k$ such that  $Delivered_j[k] < M_j[i,k,j]$. Since all communication channels are FIFO and reliable, eventually the message sent by $p_k$ to $p_j$ are received and $Delivered_j[k]$ will be equal to $M_j[i,k,j]$. Then, $p_j$ will deliver $m$. Therefore liveness is ensured by algorithm \ref{alg:bcb} in a failure free setting.
    
\end{itemize}

In a Byzantine setting, we have:

\begin{itemize}
    
    
    \item \textbf{Safety:} 
    
    \medskip
    
    \item \textbf{Liveness:} In order to implement an attack on liveness of the system, a Byzantine process $p_j$ will have to record messages that have never been sent ($p_j$ does not intend to send them) in the control matrix stored at at least one correct process $p_k$, so that $p_k$ stops delivering messages from all other correct processes. This can \textit{only} be achieved if $p_j$ successfully broadcasts the tuple $\langle j,k,sent \rangle$. But no process will deliver this broadcast without receiving a confirmation from $p_i$ in the form of an $echo$ message. Since $p_i$ is a correct process, it will broadcast a $veto$ message (instead of an $echo$ message) leading to the termination of the the false broadcast. Thus, no false messages will be recorded in the control matrix at any correct process. Therefore liveness is ensured by algorithm \ref{alg:bcb} in a Byzantine setting.
    
    
    
    
    
\end{itemize}




\end{proof}


\end{section}

==> 05-solution2.tex <==
\begin{section}{$O(n)$ space and time solution for failure free model}

In this section we present a protocol that causally orders point-to-point messages in a asynchronous failure free system. The space, time and control information complexity is $O(n)$. This protocol may require $O(n)$ control messages per message received in the worst case scenario. Each process $p_i$ maintains a vector clock $V_i$. $V_i[k]$ counts the total number of messages sent by $p_k$ as known to $p_i$. Each process $p_i$ counts the number of  messages sent overall (regardless of destination) and stores it in $V_i[i]$. The $send(j,m,V_i)$ primitive sends message $m$ with timestamp $V_i$ to process $p_j$. FIFO channels are assumed in the algorithm.


\medskip

\begin{algorithm}[H]

\SetAlgoLined

\SetKwComment{Comment}{$\triangleright$ }{}
\KwData{Each $p_i$ maintains $V_i[1...n]$ initialized to $0$ for all indices and set $S$ is initialized to $\phi$}

\medskip

Each process $p_i$ for $0 \leq i < n$ executes the following: 

\medskip

\textbf{when} message $m$ is ready to be sent to $p_j$: \\

\Indp

$V_i[i] = V_i[i] + 1$ \\
$send(j,V_i,m)$

\Indm

\medskip

\textbf{when} message $m$ is received from $p_j$: \\

\Indp
If one or more messages from $p_j$ have been received but not delivered, wait until they are delivered \\
$S_m \leftarrow \phi$

\For{$x = 0$ to $(n-1)$}{

\If{$x == j$}{Skip to the next iteration of the loop}

\If{$V_m[x] > V_i[x] + 1
$}{

$S_m \leftarrow S_m \cup \{x\}$

}


}

\For{each $y \in S$}{

$send(y,PROBE(m),-)$

}

\While{$\|S_m\| \neq 0$}{

wait for responses to arrive for all probe messages


}

\If{$\|S\| == 0$}{

$V_i \leftarrow Merge(V_i,V_m)$ \\

\textbf{deliver} $m$

}

\Indm

\medskip

\textbf{when} $PROBE(m)$ arrives from $p_j$:

\Indp

$send(j,PROBE\_RESPONSE(m),-)$

\Indm


\medskip

\textbf{when} $PROBE\_RESPONSE(m)$ arrives from $p_j$:

\Indp

$S_m \leftarrow S_m - \{j\}$

\Indm

 
\caption{CO P2P Protocol for Failure Free Systems}
\label{alg:co_ff}
\end{algorithm}







\end{section}

==> 06-impossibility_proof.tex <==
\begin{section}{Impossibility Proof}

In order to track causality in a distributed system, some form of a logical clock is required to order messages (or events) by utilizing timestamps at the receiving process. Traditionally, logical clocks use control information attached to each incoming message for update operations.
A count of the number of messages that have been sent by each process to every other process in the causal past of a message $m$ is required to determine whether it is safe to deliver $m$ without violating causal order. This means that each process $p_i$ \textit{has to} maintain a matrix clock $M^i_{sent}$ where $M^i_{sent}[j,k]$ is a count of the number of messages sent by $p_j$ to $p_k$ as known to $p_i$. Each message $m$ sent by $p_i$ is timestamped with the value of $M^i_{sent}$ at the time of sending $m$. However, in case there is a single Byzantine node $p_j$ in in an asynchronous system, it can change the values  of $M^j_{sent}$ at the time of sending $m$ to $p_i$. This may result in safety or liveness violations when $p_i$ communicates with a third process $p_k$. Lemma \ref{lemma:control} proves that appended control information can lead to liveness attacks in asynchronous systems with Byzantine nodes.  Lemma \ref{lemma:control2} shows that control information cannot be appended to messages as a result of lemma \ref{lemma:control}.

Since we are not using logical clocks to capture causality, it is not possible to ensure causal delivery of messages at the receiver's end. Therefore, constraints on when the sending process can send messages need to be enforced to maintain causal delivery of messages. Each process would need to wait to get an acknowledgement from the receiver before sending the next message. Messages would get delivered in FIFO order at the receiver. While waiting for an acknowledgment, each process would continue to receive and deliver messages. This is important to maintain concurrency and avoid deadlocks.
This can be implemented by using non-blocking synchronous sends, with the added constraint that all send events are \textit{atomic} with respect to each other.

However, lemma \ref{lemma:synch} proves that even this approach would fail in the presence of one or more Byzantine nodes.  Lemma \ref{lemma:bco} shows that the Byzantine happens before relation defined in section 2 cannot be tracked as a result of  lemmas \ref{lemma:control2} and \ref{lemma:synch}. Theorem \ref{Theorem:impossible} puts all these results together and proves that it is impossible to causally order messages in an asynchronous system with one or more Byzantine nodes.


\begin{lemma}


In a message passing system where control information is appended to every message for causality tracking, a single Byzantine node can corrupt the logical clock of every correct node and execute attacks on liveness.

\label{lemma:control}

\end{lemma}

\begin{proof}

Each message $m$ sent to $p_i$ is accompanied with a \textit{logical timestamp} in the form of a matrix clock providing an encoding of $P(m)$. Based on the definition of $\xrightarrow{B}$, it is required that the encoding of $P(m)$ maintains an entry to count the number of messages sent by $p_i$ to $p_j$, $\forall p_i,p_j \in P$.  Such an encoding will consist of a total of $n^2$ entries, $n$ entries per process. Therefore, in order to ensure that all messages $m^\prime$ $\in$ $P(m)$ whose destination is $p_i$ are delivered at $p_i$ before $m$, a matrix clock is required to encode $P(m)$. Let the matrix clock at $p_i$ be $M^i_{sent}$ where $M^i_{sent}[j,k]$ is a count of the number of messages sent by $p_j$ to $p_k$ as known to $p_i$. The protocol for ordering messages using a matrix clock is as follows:

\begin{enumerate}
    \item Each process $p_i$ maintains a vector $Delivered_i$ of size $n$ with $Delivered_i[j]$ storing a count of messages sent by $p_j$ and delivered by $p_i$. 
    
    \medskip
    
    \item Each message $m$ has an associated a matrix timestamp $M^m_{sent}$, where $M^m_{sent}$ is the matrix clock at $p_i$ at the time of sending $m$.
    
    \medskip
    
    \item When message $m$ is received by $p_i$, it is not delivered until the following condition is met:
    
    
    
    \begin{center}
    
    $\forall k$, $M^m_{sent}[k,i] \leq Delivered_i[k]$
        
    \end{center}
    
    \medskip
    
    \item After delivering a message $m$, $p_i$ merges the logical timestamp associated with $m$ with its own matrix clock, $M^i_{sent}$.
    
    
    
  
\end{enumerate}

Prior to delivering $m$ sent by $p_k$, $p_i$ will have to check that it is not merging Byzantine/malicious information from $M^m_{sent}$ into $M^i_{sent}$. We can consider $M^m_{sent}$ to be a set of $n$ vectors with the $j^{th}$ vector, $M^m_{sent}[j,*]$ being a count of the number of messages $p_j$ has sent to every process in the system. In order to make sure that $p_k$ has not artificially increased $M^m_{sent}[j,*]$ with the intention of executing an attack on liveness, $p_i$ will have to receive the current values of $M^j_{sent}[j,*]$ from $p_j$. This will put an upper bound on the amount of boosting that $p_k$ can do on $M^m_{sent}[j,*]$ and prevent an attack on liveness because the boosting is limited to the actual messages that $p_j$ has sent. This will have to be repeated for all processes. However, even after checking with every other process, if $p_k$ is Byzantine it can still boost the values of $M^m_{sent}[k,*]$ and $p_i$ would have no way to place an upper bound on $M^m_{sent}[k,*]$. It is important to note that no process knows which processes are Byzantine. Therefore, it is impossible for $p_i$ or any other process to prevent corruption of its logical clock. This argument extends to every other correct process and therefore the system is open to liveness attacks in the presence of a single Byzantine node. This concludes the proof of the lemma. $\square$




\end{proof}



\begin{lemma}

\label{lemma:control2}

Control Information cannot be appended to messages for the purpose of causally ordering messages in an asynchronous system with one or more Byzantine nodes.


\end{lemma}

\begin{proof}

From lemma \ref{lemma:control}, we know that matrix clocks are required to causally order point-to-point messages. The main takeaway from lemma \ref{lemma:control} is that a correct node cannot be certain that control information in the form of a matrix timestamp sent by another process is correct, and therefore cannot update its own matrix clock and guarantee its correctness. Therefore, an asynchronous system with even a single Byzantine fault cannot append control information to messages for the purpose of causally ordering messages. $\square$

\end{proof}




\begin{lemma}
\label{lemma:synch}

Non-blocking asynchronous sends that are atomic with respect to each other can implement safety at the expense of liveness when messages are delivered in FIFO order of arrival.

\end{lemma}




\begin{proof}


In order to ensure safety, whenever messages $m$ and $m'$ arrive at correct process $p_i$ and $m \xrightarrow{B} m'$, $m$ must arrive before $m'$. This is because $p_i$ delivers messages in FIFO order. The causal relationship between $m$ and $m'$ may be due to the following reasons:

\begin{enumerate}
    \item Any (correct or faulty) process $p_j$ sends $m$ and then $m'$ to $p_i$. Since we have FIFO channels, $m$ will arrive before $m'$ at $p_i$ ensuring safety.
    
    \medskip
    
    \item Any correct process $p_j$ sends $m$ to correct process $p_i$, then sends $m''$ to correct process $p_k$. After $p_k$ delivers $m''$, $p_k$ sends $m'$ to $p_i$. Since all sends are synchronous and atomic with respect to each other $p_j$ will send $m''$ only after $m$ is received at $p_i$. This ensures safety because $m$ will be delivered before $m'$.
\end{enumerate}

However, if a correct process $p_i$ sends message $m$ to a Byzantine process $p_j$, $p_j$ may never acknowledge receiving $m$. This will result in $p_i$ being unable to send any further messages throughout the execution. Therefore, synchronous sends can guarantee safety at the expense of liveness. This concludes the proof of the lemma. $\square$

\end{proof}

\begin{corollary}

It is impossible to causally order events in an asynchronous system with one or more Byzantine faults by performing non-blocking synchronous sends that are atomic to each other along with delivering messages in FIFO order.

\end{corollary}


\begin{lemma}



\label{lemma:bco}

The Byzantine happens before relation cannot be captured in an asynchronous system with one or more Byzantine nodes.

\end{lemma}

\begin{proof}

From lemma \ref{lemma:control2}, it is known that control information cannot be appended to messages for causally ordering messages in an asynchronous system with a single Byzantine node. Therefore, it is not possible for correct processes to update the local matrix clock. From lemma \ref{lemma:control}, Byzantine happens before relation cannot be tracked without a matrix clock. However, since matrix clocks cannot be updated, the matrix timestamps used to capture the Byzantine happens before relation will be incorrect. As a result of lemma \ref{lemma:synch}, it is not possible to causally order events by introducing virtual synchrony. Therefore, the Byzantine happens before relation cannot be captured in an asynchronous system with a single Byzantine node. $\square$


\end{proof}



\begin{theorem}

It is impossible to causally order point-to-point messages in an asynchronous message passing system with one or more Byzantine nodes.

\label{Theorem:impossible}

\end{theorem}

\begin{proof}

As a result of lemma \ref{lemma:bco}, we cannot capture the Byzantine happens before relation in an asynchronous system with one or more Byzantine nodes. It is not possible to introduce a causal ordering amongst a set of messages delivered at a process without a mechanism creating a relationship between messages ordered by some \textit{happens before relation}. Therefore, it becomes impossible to causally order messages in an asynchronous message passing system with one or more Byzantine nodes. $\square$


\end{proof}



\end{section}
